Self supervised learning improves dMMR/MSI detection from histology slides across multiple cancers

Microsatellite instability (MSI) is a tumor phenotype whose diagnosis largely impacts patient care in colorectal cancers (CRC), and is associated with response to immunotherapy in all solid tumors. Deep learning models detecting MSI tumors directly from H&E stained slides have shown promise in improving diagnosis of MSI patients. Prior deep learning models for MSI detection have relied on neural networks pretrained on ImageNet dataset, which does not contain any medical image. In this study, we leverage recent advances in self-supervised learning by training neural networks on histology images from the TCGA dataset using MoCo V2. We show that these networks consistently outperform their counterparts pretrained using ImageNet and obtain state-of-the-art results for MSI detection with AUCs of 0.92 and 0.83 for CRC and gastric tumors, respectively. These models generalize well on an external CRC cohort (0.97 AUC on PAIP) and improve transfer from one organ to another. Finally we show that predictive image regions exhibit meaningful histological patterns, and that the use of MoCo features highlighted more relevant patterns according to an expert pathologist.

==> bibli.tex <==
@article{kather2019deep,
  title={Deep learning can predict microsatellite instability directly from histology in gastrointestinal cancer},
  author={Kather, Jakob Nikolas and Pearson, Alexander T and Halama, Niels and J{\"a}ger, Dirk and Krause, Jeremias and Loosen, Sven H and Marx, Alexander and Boor, Peter and Tacke, Frank and Neumann, Ulf Peter and others},
  journal={Nature medicine},
  volume={25},
  number={7},
  pages={1054--1056},
  year={2019},
  publisher={Nature Publishing Group}
}

@article{echle2020clinical,
  title={Clinical-Grade detection of microsatellite instability in colorectal tumors by deep learning},
  author={Echle, Amelie and Grabsch, Heike Irmgard and Quirke, Philip and van den Brandt, Piet A and West, Nicholas P and Hutchins, Gordon GA and Heij, Lara R and Tan, Xiuxiang and Richman, Susan D and Krause, Jeremias and others},
  journal={Gastroenterology},
  volume={159},
  number={4},
  pages={1406--1416},
  year={2020},
  publisher={Elsevier}
}
@article{yamashita2021deep,
  title={Deep learning model for the prediction of microsatellite instability in colorectal cancer: a diagnostic study},
  author={Yamashita, Rikiya and Long, Jin and Longacre, Teri and Peng, Lan and Berry, Gerald and Martin, Brock and Higgins, John and Rubin, Daniel L and Shen, Jeanne},
  journal={The Lancet Oncology},
  volume={22},
  number={1},
  pages={132--141},
  year={2021},
  publisher={Elsevier}
}
@inproceedings{zhang2018adversarial,
  title={Adversarial deep learning for microsatellite instability prediction from histopathology slides},
  author={Zhang, Renyu and Osinski, Boleslaw L and Taxter, Timothy J and Perera, Jason and Lau, Denise J and Khan, Aly A},
  booktitle={Proceedings of the 1st Conference on Medical Imaging with Deep Learning (MIDL 2018), Amsterdam, The Netherlands},
  pages={4--6},
  year={2018}
}
@article{bilal2021novel,
  title={Novel deep learning algorithm predicts the status of molecular pathways and key mutations in colorectal cancer from routine histology images},
  author={Bilal, Mohsin and Raza, Shan E Ahmed and Azam, Ayesha and Graham, Simon and Ilyas, Muhammad and Cree, Ian A and Snead, David and Minhas, Fayyaz and Rajpoot, Nasir M},
  journal={medRxiv},
  year={2021},
  publisher={Cold Spring Harbor Laboratory Press}
}
@article{cao2020development,
  title={Development and interpretation of a pathomics-based model for the prediction of microsatellite instability in Colorectal Cancer},
  author={Cao, Rui and Yang, Fan and Ma, Si-Cong and Liu, Li and Zhao, Yu and Li, Yan and Wu, De-Hua and Wang, Tongxin and Lu, Wei-Jia and Cai, Wei-Jing and others},
  journal={Theranostics},
  volume={10},
  number={24},
  pages={11080},
  year={2020},
  publisher={Ivyspring International Publisher}
}
@article{kather2020pan,
  title={Pan-cancer image-based detection of clinically actionable genetic alterations},
  author={Kather, Jakob Nikolas and Heij, Lara R and Grabsch, Heike I and Loeffler, Chiara and Echle, Amelie and Muti, Hannah Sophie and Krause, Jeremias and Niehues, Jan M and Sommer, Kai AJ and Bankhead, Peter and others},
  journal={Nature Cancer},
  volume={1},
  number={8},
  pages={789--799},
  year={2020},
  publisher={Nature Publishing Group}
}
@article{hong2020predicting,
  title={Predicting endometrial cancer subtypes and molecular features from histopathology images using multi-resolution deep learning models},
  author={Hong, Runyu and Liu, Wenke and DeLair, Deborah and Razavian, Narges and Feny{\"o}, David},
  journal={bioRxiv},
  year={2020},
  publisher={Cold Spring Harbor Laboratory}
}
@article{lee2021feasibility,
  title={Feasibility of deep learning-based fully automated classification of microsatellite instability in tissue slides of colorectal cancer},
  author={Lee, Sung Hak and Song, In Hye and Jang, Hyun-Jong},
  journal={International Journal of Cancer},
  year={2021},
  publisher={Wiley Online Library}
}
@article{hildebrand2021artificial,
  title={Artificial Intelligence for Histology-Based Detection of Microsatellite Instability and Prediction of Response to Immunotherapy in Colorectal Cancer},
  author={Hildebrand, Lindsey A and Pierce, Colin J and Dennis, Michael and Paracha, Munizay and Maoz, Asaf},
  journal={Cancers},
  volume={13},
  number={3},
  pages={391},
  year={2021},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@article{greenson2009pathologic,
  title={Pathologic predictors of microsatellite instability in colorectal cancer},
  author={Greenson, Joel K and Huang, Shu-Chen and Herron, Casey and Moreno, Victor and Bonner, Joseph D and Tomsho, Lynn P and Ben-Izhak, Ofer and Cohen, Hector I and Trougouboff, Phillip and Bejhar, Jacob and others},
  journal={The American journal of surgical pathology},
  volume={33},
  number={1},
  pages={126},
  year={2009},
  publisher={NIH Public Access}
}
@article{jenkins2007pathology,
  title={Pathology features in Bethesda guidelines predict colorectal cancer microsatellite instability: a population-based study},
  author={Jenkins, Mark A and Hayashi, Shinichi and O’shea, Anne-Marie and Burgart, Lawrence J and Smyrk, Tom C and Shimizu, David and Waring, Paul M and Ruszkiewicz, Andrew R and Pollett, Aaron F and Redston, Mark and others},
  journal={Gastroenterology},
  volume={133},
  number={1},
  pages={48--56},
  year={2007},
  publisher={Elsevier}
}
@article{hyde2010histology,
  title={A histology-based model for predicting microsatellite instability in colorectal cancers},
  author={Hyde, Angela and Fontaine, Daniel and Stuckless, Susan and Green, Roger and Pollett, Aaron and Simms, Michelle and Sipahimalani, Payal and Parfrey, Patrick and Younghusband, Banfield},
  journal={The American journal of surgical pathology},
  volume={34},
  number={12},
  pages={1820--1829},
  year={2010},
  publisher={LWW}
}
@article{fujiyoshi2017predictive,
  title={Predictive model for high-frequency microsatellite instability in colorectal cancer patients over 50 years of age},
  author={Fujiyoshi, Kenji and Yamaguchi, Tatsuro and Kakuta, Miho and Takahashi, Akemi and Arai, Yoshiko and Yamada, Mina and Yamamoto, Gou and Ohde, Sachiko and Takao, Misato and Horiguchi, Shin-ichiro and others},
  journal={Cancer medicine},
  volume={6},
  number={6},
  pages={1255--1263},
  year={2017},
  publisher={Wiley Online Library}
}
@article{roman2010microsatellite,
  title={Microsatellite instability of the colorectal carcinoma can be predicted in the conventional pathologic examination. A prospective multicentric study and the statistical analysis of 615 cases consolidate our previously proposed logistic regression model},
  author={Rom{\'a}n, Ruth and Verd{\'u}, Montse and Calvo, Miquel and Vidal, August and Sanjuan, Xavier and Jimeno, Mireya and Salas, Antonio and Autonell, Josefina and Trias, Isabel and Gonz{\'a}lez, Marta and others},
  journal={Virchows Archiv},
  volume={456},
  number={5},
  pages={533--541},
  year={2010},
  publisher={Springer}
}
@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}
@article{dehaene2020self,
  title={Self-Supervision Closes the Gap Between Weak and Strong Supervision in Histology},
  author={Dehaene, Olivier and Camara, Axel and Moindrot, Olivier and de Lavergne, Axel and Courtiol, Pierre},
  journal={arXiv preprint arXiv:2012.03583},
  year={2020}
}
@article{prasad2018cancer,
  title={Cancer drugs approved based on biomarkers and not tumor type—FDA approval of pembrolizumab for mismatch repair-deficient solid cancers},
  author={Prasad, Vinay and Kaestner, Victoria and Mailankody, Sham},
  journal={JAMA oncology},
  volume={4},
  number={2},
  pages={157--158},
  year={2018},
  publisher={American Medical Association}
}
@article{le2017mismatch,
  title={Mismatch repair deficiency predicts response of solid tumors to PD-1 blockade},
  author={Le, Dung T and Durham, Jennifer N and Smith, Kellie N and Wang, Hao and Bartlett, Bjarne R and Aulakh, Laveet K and Lu, Steve and Kemberling, Holly and Wilt, Cara and Luber, Brandon S and others},
  journal={Science},
  volume={357},
  number={6349},
  pages={409--413},
  year={2017},
  publisher={American Association for the Advancement of Science}
}
@article{svrcek2019msi,
  title={MSI/MMR-deficient tumor diagnosis: Which standard for screening and for diagnosis? Diagnostic modalities for the colon and other sites: Differences between tumors},
  author={Svrcek, Magali and Lascols, Olivier and Cohen, Romain and Collura, Ada and Jonch{\`e}re, Vincent and Fl{\'e}jou, Jean-Fran{\c{c}}ois and Buhard, Olivier and Duval, Alex},
  journal={Bulletin du cancer},
  volume={106},
  number={2},
  pages={119--128},
  year={2019},
  publisher={Elsevier}
}
@article{sargent2010defective,
  title={Defective mismatch repair as a predictive marker for lack of efficacy of fluorouracil-based adjuvant therapy in colon cancer},
  author={Sargent, Daniel J and Marsoni, Silvia and Monges, Genevieve and Thibodeau, Stephen N and Labianca, Roberto and Hamilton, Stanley R and French, Amy J and Kabat, Brian and Foster, Nathan R and Torri, Valter and others},
  journal={Journal of Clinical Oncology},
  volume={28},
  number={20},
  pages={3219},
  year={2010},
  publisher={American Society of Clinical Oncology}
}

@inproceedings{deng2009imagenet,
  title={Imagenet: A large-scale hierarchical image database},
  author={Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Li, Kai and Fei-Fei, Li},
  booktitle={2009 IEEE conference on computer vision and pattern recognition},
  pages={248--255},
  year={2009},
  organization={Ieee}
}
@article{chen2020big,
  title={Big self-supervised models are strong semi-supervised learners},
  author={Chen, Ting and Kornblith, Simon and Swersky, Kevin and Norouzi, Mohammad and Hinton, Geoffrey},
  journal={arXiv preprint arXiv:2006.10029},
  year={2020}
}
@article{caron2020unsupervised,
  title={Unsupervised learning of visual features by contrasting cluster assignments},
  author={Caron, Mathilde and Misra, Ishan and Mairal, Julien and Goyal, Priya and Bojanowski, Piotr and Joulin, Armand},
  journal={arXiv preprint arXiv:2006.09882},
  year={2020}
}
@inproceedings{he2020momentum,
  title={Momentum contrast for unsupervised visual representation learning},
  author={He, Kaiming and Fan, Haoqi and Wu, Yuxin and Xie, Saining and Girshick, Ross},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={9729--9738},
  year={2020}
}
@article{chen2020improved,
  title={Improved baselines with momentum contrastive learning},
  author={Chen, Xinlei and Fan, Haoqi and Girshick, Ross and He, Kaiming},
  journal={arXiv preprint arXiv:2003.04297},
  year={2020}
}
@article{lu2019semi,
  title={Semi-supervised histology classification using deep multiple instance learning and contrastive predictive coding},
  author={Lu, Ming Y and Chen, Richard J and Wang, Jingwen and Dillon, Debora and Mahmood, Faisal},
  journal={arXiv preprint arXiv:1910.10825},
  year={2019}
}
@article{koohbanani2021self,
  title={Self-Path: Self-supervision for Classification of Pathology Images with Limited Annotations},
  author={Koohbanani, Navid Alemi and Unnikrishnan, Balagopal and Khurram, Syed Ali and Krishnaswamy, Pavitra and Rajpoot, Nasir},
  journal={IEEE Transactions on Medical Imaging},
  year={2021},
  publisher={IEEE}
}
@article{courtiol2018classification,
  title={Classification and disease localization in histopathology using only global labels: A weakly-supervised approach},
  author={Courtiol, Pierre and Tramel, Eric W and Sanselme, Marc and Wainrib, Gilles},
  journal={arXiv preprint arXiv:1802.02212},
  year={2018}
}
@inproceedings{ilse2018attention,
  title={Attention-based deep multiple instance learning},
  author={Ilse, Maximilian and Tomczak, Jakub and Welling, Max},
  booktitle={International conference on machine learning},
  pages={2127--2136},
  year={2018},
  organization={PMLR}
}

@inproceedings{li2021dual,
  title={Dual-stream multiple instance learning network for whole slide image classification with self-supervised contrastive learning},
  author={Li, Bin and Li, Yin and Eliceiri, Kevin W},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={14318--14328},
  year={2021}
}
@article{gildenblat2019self,
  title={Self-supervised similarity learning for digital pathology},
  author={Gildenblat, Jacob and Klaiman, Eldad},
  journal={arXiv preprint arXiv:1905.08139},
  year={2019}
}
@inproceedings{abbet2021self,
  title={Self-Rule to Adapt: Learning Generalized Features from Sparsely-Labeled Data Using Unsupervised Domain Adaptation for Colorectal Cancer Tissue Phenotyping},
  author={Abbet, Christian and Studer, Linda and Fischer, Andreas and Dawson, Heather and Zlobec, Inti and Bozorgtabar, Behzad and Thiran, Jean-Philippe},
  booktitle={Medical Imaging with Deep Learning},
  year={2021}
}
@article{srinidhi2021self,
  title={Self-supervised driven consistency training for annotation efficient histopathology image analysis},
  author={Srinidhi, Chetan L and Kim, Seung Wook and Chen, Fu-Der and Martel, Anne L},
  journal={arXiv preprint arXiv:2102.03897},
  year={2021}
}
@inproceedings{chen2020simple,
  title={A simple framework for contrastive learning of visual representations},
  author={Chen, Ting and Kornblith, Simon and Norouzi, Mohammad and Hinton, Geoffrey},
  booktitle={International conference on machine learning},
  pages={1597--1607},
  year={2020},
  organization={PMLR}
}
@article{chen2021empirical,
  title={An empirical study of training self-supervised vision transformers},
  author={Chen, Xinlei and Xie, Saining and He, Kaiming},
  journal={arXiv preprint arXiv:2104.02057},
  year={2021}
}
@article{grill2020bootstrap,
  title={Bootstrap your own latent: A new approach to self-supervised learning},
  author={Grill, Jean-Bastien and Strub, Florian and Altch{\'e}, Florent and Tallec, Corentin and Richemond, Pierre H and Buchatskaya, Elena and Doersch, Carl and Pires, Bernardo Avila and Guo, Zhaohan Daniel and Azar, Mohammad Gheshlaghi and others},
  journal={arXiv preprint arXiv:2006.07733},
  year={2020}
}
@article{li2021efficient,
  title={Efficient Self-supervised Vision Transformers for Representation Learning},
  author={Li, Chunyuan and Yang, Jianwei and Zhang, Pengchuan and Gao, Mei and Xiao, Bin and Dai, Xiyang and Yuan, Lu and Gao, Jianfeng},
  journal={arXiv preprint arXiv:2106.09785},
  year={2021}
}
@article{caron2021emerging,
  title={Emerging properties in self-supervised vision transformers},
  author={Caron, Mathilde and Touvron, Hugo and Misra, Ishan and J{\'e}gou, Herv{\'e} and Mairal, Julien and Bojanowski, Piotr and Joulin, Armand},
  journal={arXiv preprint arXiv:2104.14294},
  year={2021}
}
@article{ciga2020self,
  title={Self supervised contrastive learning for digital histopathology},
  author={Ciga, Ozan and Martel, Anne L and Xu, Tony},
  journal={arXiv preprint arXiv:2011.13971},
  year={2020}
}
@inproceedings{sikaroudi2020supervision,
  title={Supervision and source domain impact on representation learning: A histopathology case study},
  author={Sikaroudi, Milad and Safarpoor, Amir and Ghojogh, Benyamin and Shafiei, Sobhan and Crowley, Mark and Tizhoosh, Hamid R},
  booktitle={2020 42nd Annual International Conference of the IEEE Engineering in Medicine \& Biology Society (EMBC)},
  pages={1400--1403},
  year={2020},
  organization={IEEE}
}
@article{dipalma2021resolution,
  title={Resolution-Based Distillation for Efficient Histology Image Classification},
  author={DiPalma, Joseph and Suriawinata, Arief A and Tafe, Laura J and Torresani, Lorenzo and Hassanpour, Saeed},
  journal={arXiv preprint arXiv:2101.04170},
  year={2021}
}
@article{tajbakhsh2020embracing,
  title={Embracing imperfect datasets: A review of deep learning solutions for medical image segmentation},
  author={Tajbakhsh, Nima and Jeyaseelan, Laura and Li, Qian and Chiang, Jeffrey N and Wu, Zhihao and Ding, Xiaowei},
  journal={Medical Image Analysis},
  volume={63},
  pages={101693},
  year={2020},
  publisher={Elsevier}
}
@article{colaprico2016tcgabiolinks,
  title={TCGAbiolinks: an R/Bioconductor package for integrative analysis of TCGA data},
  author={Colaprico, Antonio and Silva, Tiago C and Olsen, Catharina and Garofano, Luciano and Cava, Claudia and Garolini, Davide and Sabedot, Thais S and Malta, Tathiane M and Pagnotta, Stefano M and Castiglioni, Isabella and others},
  journal={Nucleic acids research},
  volume={44},
  number={8},
  pages={e71--e71},
  year={2016},
  publisher={Oxford University Press}
}
@article{delong1988comparing,
  title={Comparing the areas under two or more correlated receiver operating characteristic curves: a nonparametric approach},
  author={DeLong, Elizabeth R and DeLong, David M and Clarke-Pearson, Daniel L},
  journal={Biometrics},
  pages={837--845},
  year={1988},
  publisher={JSTOR}
}
@article{sun2014fast,
  title={Fast implementation of DeLong’s algorithm for comparing the areas under correlated receiver operating characteristic curves},
  author={Sun, Xu and Xu, Weichao},
  journal={IEEE Signal Processing Letters},
  volume={21},
  number={11},
  pages={1389--1393},
  year={2014},
  publisher={IEEE}
}
@article{kacew2021artificial,
  title={Artificial intelligence can cut costs while maintaining accuracy in colorectal cancer genotyping},
  author={Kacew, Alec J and Strohbehn, Garth W and Saulsberry, Loren and Laiteerapong, Neda and Cipriani, Nicole A and Kather, Jakob N and Pearson, Alexander T},
  journal={Frontiers in Oncology},
  volume={11},
  year={2021},
  publisher={Frontiers Media SA}
}
@inproceedings{ronneberger2015u,
  title={U-net: Convolutional networks for biomedical image segmentation},
  author={Ronneberger, Olaf and Fischer, Philipp and Brox, Thomas},
  booktitle={International Conference on Medical image computing and computer-assisted intervention},
  pages={234--241},
  year={2015},
  organization={Springer}
}
@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}
@article{luchini2019esmo,
  title={ESMO recommendations on microsatellite instability testing for immunotherapy in cancer, and its relationship with PD-1/PD-L1 expression and tumour mutational burden: a systematic review-based approach},
  author={Luchini, C and Bibeau, F and Ligtenberg, MJL and Singh, N and Nottegar, A and Bosse, T and Miller, R and Riaz, N and Douillard, J-Y and Andre, F and others},
  journal={Annals of Oncology},
  volume={30},
  number={8},
  pages={1232--1243},
  year={2019},
  publisher={Elsevier}
}
@article{dosovitskiy2020image,
  title={An image is worth 16x16 words: Transformers for image recognition at scale},
  author={Dosovitskiy, Alexey and Beyer, Lucas and Kolesnikov, Alexander and Weissenborn, Dirk and Zhai, Xiaohua and Unterthiner, Thomas and Dehghani, Mostafa and Minderer, Matthias and Heigold, Georg and Gelly, Sylvain and others},
  journal={arXiv preprint arXiv:2010.11929},
  year={2020}
}

